Streaming Algorithms for Learning with Experts: Deterministic Versus Robust

In the online learning with experts problem, an algorithm must make a prediction about an outcome on each of $T$ days (or times), given a set of $n$ experts who make predictions on each day (or time). The algorithm is given feedback on the outcomes of each day, including the cost of its prediction and the cost of the expert predictions, and the goal is to make a prediction with the minimum cost, specifically compared to the best expert in the set. Recent work by Srinivas, Woodruff, Xu, and Zhou (STOC 2022) introduced the study of the online learning with experts problem under memory constraints. However, often the predictions made by experts or algorithms at some time influence future outcomes, so that the input is adaptively chosen. Whereas deterministic algorithms would be robust to adaptive inputs, existing algorithms all crucially use randomization to sample a small number of experts. In this paper, we study deterministic and robust algorithms for the experts problem. We first show a space lower bound of $\widetilde{\Omega}\left(\frac{nM}{RT}\right)$ for any deterministic algorithm that achieves regret $R$ when the best expert makes $M$ mistakes. Our result shows that the natural deterministic algorithm, which iterates through pools of experts until each expert in the pool has erred, is optimal up to polylogarithmic factors. On the positive side, we give a randomized algorithm that is robust to adaptive inputs that uses $\widetilde{O}\left(\frac{n}{R\sqrt{T}}\right)$ space for $M=O\left(\frac{R^2 T}{\log^2 n}\right)$, thereby showing a smooth space-regret trade-off.

==> apx.tex <==
\section{Tools from Differential Privacy}
Our algorithmic results rely on the following tools from differential privacy.
\begin{definition}[Differential privacy, \cite{DworkMNS06}]
Given a privacy parameter $\eps>0$ and a failure parameter $\delta\in(0,1)$, a randomized algorithm $\calA:\calX^*\to\calY$ is $(\eps,\delta)$-differentially private if, for every pair of neighboring streams $S$ and $S'$ and for all $E\subseteq\calY$,
\[\PPr{\calA(S)\in E}\le e^{\eps}\cdot\PPr{\calA(S')\in E}+\delta.\]
\end{definition}

%\begin{theorem}[Amplification via sampling, e.g.,~\cite{BunNSV15}]
%\label{thm:dp:sampling}
%Given a privacy parameter $\eps>0$ and a failure parameter $\delta\in(0,1)$, let $\calA$ be an $(\eps,\delta)$-differentially private algorithm. 
%Given a database $S$ of size $n$, let $\calA'$ be the algorithm that constructs a database $T\subset S$ by subsampling (with replacement) $s\le\frac{n}{2}$ rows of $S$ and outputs $\calA(T)$. 
%Then $\calA'$ is $(\eps',\delta')$-differentially private for
%\[\eps'=\frac{6\eps k}{n},\qquad\delta'=\exp(6\eps k/n)\,\frac{4k\delta}{n}.\]
%\end{theorem}

\begin{theorem}[Private median, e.g.,~\cite{HassidimKMMS20}]
\label{thm:dp:median}
Given a database $\calD\in X^*$, a privacy parameter $\eps>0$ and a failure parameter $\delta\in(0,1)$, there exists an $(\eps,0)$-differentially private algorithm $\privmed$ that outputs an element $x\in X$ such that with probability at least $1-\delta$, there are at least $\frac{|S|}{2}-m$ elements in $S$ that are at least $x$, and at least $\frac{|S|}{2}-m$ elements in $S$ in $S$ that are at most $x$, for $m=\O{\frac{1}{\eps}\log\frac{|X|}{\delta}}$. 
\end{theorem}

\begin{theorem}[Advanced composition, e.g.,~\cite{DworkRV10}]
\label{thm:adaptive:queries}
Let $\eps,\delta'\in(0,1]$ and let $\delta\in[0,1]$. 
Any mechanism that permits $k$ adaptive interactions with mechanisms that preserve $(\eps,\delta)$-differential privacy guarantees $(\eps',k\delta+\delta')$-differential privacy, where $\eps'=\sqrt{2k\ln\frac{1}{\delta'}}\cdot\eps+2k\eps^2$. 
\end{theorem}

\begin{theorem}[Generalization of DP, e.g.,~\cite{DworkFHPRR15,BassilyNSSSU21}]
\label{thm:generalization}
Let $\eps\in(0,1/3)$, $\delta\in(0,\eps/4)$, and $n\ge\frac{1}{\eps^2}\log\frac{2\eps}{\delta}$. 
Suppose $\calA:X^n\to 2^X$ is an $(\eps,\delta)$-differentially private algorithm that curates a database of size $n$ and produces a function $h:X\to\{0,1\}$. 
Suppose $\calD$ is a distribution over $X$ and $S$ is a set of $n$ elements drawn independently and identically distributed from $\calD$. 
Then
\[\PPPr{S\sim\calD,h\gets\calA(S)}{\left|\frac{1}{|S|}\sum_{x\in S}h(x)-\EEx{x\sim\calD}{h(x)}\right|\ge10\eps}<\frac{\delta}{\eps}.\]
\end{theorem}



\section{Proof of the Single-Coordinate Information Cost Lower Bound}\label{sec:key-lemma-pf}
We now show the single-coordinate lower bound of \autoref{lem:single-lb}.
\begin{proof}[Proof of \autoref{lem:single-lb}]
Consider a protocol that is correct with probability $1-2^{-\Theta(T)}$ and let $(C_1,C_2,\ldots , C_T) \sim \zeta^T$ be a single column drawn from the NO case, where each coordinate is i.i.d.\ Bernoulli with parameter $1/2$. For notational convenience, let $\Pi = \Pi (C_1,\cdots , C_T)$ denote the transcript given the input $(C_1,C_2,\cdots , C_T)$.   We consider the one-way message-passing model, where each player $P_i$ holds the input $C_i$. For all $i<T$, let $M_i$ denote the message sent from player $P_i$ to player $P_{i+1}$.   

By the chain rule of mutual information, the information cost of the transcript,  the left-side of \autoref{eqn:single-coord-ic} that we need to bound, can be written as 
\begin{align}
     I(\Pi; C_1,C_2,\ldots, C_T) =  \sum_{j= 1}^{T} I\left(M_j ;  C_1,C_2,\ldots, C_T \mid  M_{<j}\right).
\end{align}
By the independence of one-way communication,  we have
\begin{align}
    I\left(M_j ;  C_1,C_2,\ldots, C_T \mid  M_{<j}\right) = I\left(M_j ;  C_j \mid  M_{<j}\right).
\end{align}
Combining the two equalities above, the information cost equals
\begin{equation}\label{eqn:ic-24}
     I(\Pi; C_1,C_2,\ldots, C_T) = \sum_{j=1}^T  I\left(M_j ;  C_j \mid  M_{<j}\right).
\end{equation}
We  now lower bound the right-side. First, we make the following definition.
For any $i \in [T]$, we say that $(M_i, M_{< i})$ is \textit{informative} (for $i$) if 
\begin{equation}
   \left| \Pr (C_i = 0  \mid M_i, M_{< i} ) -  \Pr (C_i = 1  \mid M_i, M_{< i} ) \right| \geq c
\end{equation}
for some constant $c > 0$; and uninformative otherwise. 
Intuitively, an informative  $(M_i, M_{< i})$  means that conditional on the past messages $ M_{< i}$,  the message $M_i$ reveals much information about $C_i$.  
Hence, in this case, $I(M_i, C_i \mid M_{< i})$ would be large. 
Now for all $i\in [T]$, let $p_i $ be the probability that $(M_i, M_{< i})$ is  informative (for $i$). 

Conceptually, we   need to show that $\sum_i p_i$ is large, since then there would be sufficiently many informative  messages, and so the information cost in the left-side of \autoref{eqn:ic-24} is high. We formalize this idea in the following lemma.
\begin{lemma}\label{lem:ic-sum-pj}
In the setting above, where $c >0$ is a constant, the information cost can be lower bounded by 
\begin{align}\label{eqn:sum-ic-26}
  I(\Pi; C_1,C_2,\ldots, C_T) = \sum_{j=1}^T  I\left(M_j ;  C_j \mid  M_{<j}\right) \geq \Omega \left(\sum_{j=1}^T p_j\right)
\end{align}
\end{lemma}
\begin{proof}
We start by  expanding the definition of the mutual information terms. For each  $j \in T$, we have 
\begin{align}\label{eqn:def-ci-27}
     I\left(M_j ;  C_j \mid  M_{<j}\right) &= H\left(C_j \mid M_{<j} \right) - H\left(C_j \mid M_j, M_{<j}\right)
\end{align}
For the first term, notice that $C_j$ and $M_{<j}$ are independent by one-way communication. Moreover, by definition $C_j$ is Bernoulli with parameter $1/2$. Therefore, \[H(C_j \mid M_{<j}) = H(C_j) = H(1/2) = 1.\]  
For the second term, 
\begin{itemize}
    \item either $(M_j, M_{<j})$ is informative, which holds with probability $p_j$, and in this case, the conditional entropy is upper bounded by $ H\left(C_j \mid M_j, M_{<j}\right) \leq H(1/2 + c/2)$; 
    \item or $(M_j, M_{<j})$ is uninformative, and in this case, we trivially upper bound the conditional entropy by $ H\left(C_j \mid M_j, M_{<j}\right) \leq 1$; 
\end{itemize} 
Putting the observations together and using  \autoref{eqn:def-ci-27}, it follows   that 
\begin{align*}
    I\left(M_j ;  C_j \mid  M_{<j}\right) &=H\left(C_j \mid M_{<j} \right) - H\left(C_j \mid M_j, M_{<j}\right)\\
%    I\left(C_j \mid M_j, M_{<j}\right) &=H\left(C_j \mid M_{<j} \right) - H\left(C_j \mid M_j, M_{<j}\right)\\
    &\ge 1 - (p_j \cdot H(1/2 + c/2) + (1-p_j) \cdot 1) \\
    &= p_j - p_j \cdot H(1/2 + c/2)\\
    &\ge p_j  \left(1- \sqrt{1-c^2}\right)\\
    &\ge c^2\cdot  \Omega(p_j),
\end{align*}
where the second last step uses the upper bound of Lemma \ref{lem:entropy-bound} and the last step follows since $1-\sqrt{1-x^2} \geq x^2/5$ for $x\in [0,1]$.
Summing over $j = 1,2,\ldots, T$ in \autoref{eqn:sum-ic-26} finishes the proof.
\end{proof}
To prove the claimed information cost inequality \autoref{eqn:single-coord-ic}, we show that $\sum_i p_i = \Omega(M)$. 
%Suppose for the sake of a contradiction that    $\sum_i p_i = o(M)$.  Then by a Markov bound on the random input bits $(C_i)_{i=1}^T$ of all the players, there are $o(M)$ players for
%which they send a message $M_i$ such that $(M_i , M_{<i})$ is informative, given the previous messages $M_{<i}$.

\begin{lemma}\label{lem:sum-pj}
There exists a constant $\gamma>0$ such that 
\[\sum_{j=1}^T p_j>\gamma\cdot M.\]
\end{lemma}
\begin{proof}
Suppose by way of contradiction that $\sum_{j=1}^T p_j=o(M)$. 
Let $A$ be a protocol that sends (possibly random) messages $M_1,\ldots,M_T$ on a random input $C\in\{0,1\}^T\sim\zeta^T$ drawn uniformly from the NO distribution, i.e., each coordinate of $C:=C_1,\ldots,C_T$ is picked to be $0$ with probability $\frac{1}{2}$ and $1$ with probability $\frac{1}{2}$. 
Moreover, suppose $A$ is a protocol that distinguishes between a YES instance and a NO instance with probability at least $1-\frac{e^{-cT}2^{-T}}{8}$, for some constant $c>0$. 

Since $p_i$ is the probability that $M_i$ is informative, then by assumption, the expected number of informative indices $i$ over the messages $M_1,\ldots,M_T$ is $f(M)$ for some $f(M)=o(M)$. 
Thus by Markov's inequality, the probability that the number of informative indices is at most $10f(M)=o(M)$ with probability at least $\frac{9}{10}$. 
Let $S$ be the set of the uninformative indices so that $|S|=T-10f(M)=T-o(M)$. 
Let $C'$ be an input that agrees with $C$ on the informative indices $[T]\setminus S$ and is chosen arbitrarily on uninformative indices $S$, so that $C'_i=C_i$ for $i\in[T]\setminus S$. 
 
By definition, each uninformative index only changes the distribution of the output by a $(1\pm c)$ factor. 
In particular, for $c\in(0,1/2)$, the probability that the protocol $A$ generates $\Pi$ on input $C'$ is at least $(1-c)^T\ge e^{-2cT}$ times the probability that the protocol $A$ generates $\Pi$ on input $C$. 
However, since $C$ can differ from $C'$ on $S$, then $C$ can differ from $C'$ on $|S|=T-10f(M)=T-o(M)$ indices. 

Now since each coordinate of $C$ is picked to be $0$ with probability $\frac{1}{2}$ and $1$ with probability $\frac{1}{2}$, then the probability that $C$ contains more than $T-M$ zeros is at least $1-T^M\cdot\frac{1}{2^T}\ge 1-2^{T/2}$ for sufficiently large $T$. 
But then there exists a choice of $C'$ that contains fewer than $\frac{M}{2}$ zeros such that $A$ will also output $\Pi$ with probability at least $\frac{e^{-cT}}{2}$. 
Since $C'$ contains fewer than $\frac{M}{2}$, then $C'$ is more likely to generated from a YES instance and indeed a YES instance will generate $C$ with probability $2^{-T}$. 
On the other hand, since $\Pi$ corresponds to a transcript for which $A$ will output NO, then the probability that $A$ is incorrect on $C'$ is at least $\frac{e^{-cT}}{4}$, which contradicts the claim that $A$ succeeds with probability $1-\frac{e^{-cT}2^{-T}}{8}$. 
Thus it follows that $\sum_{j=1}^T p_j=\Omega(M)$, as desired.  
\end{proof}

Now we combine Lemma \ref{lem:ic-sum-pj} and Lemma \ref{lem:sum-pj}. This implies that the information cost can be lower bounded by
\begin{equation}
     I(\Pi; C_1,C_2,\ldots, C_T) \geq  \Omega \left(\sum_{j=1}^T p_j\right) \geq \gamma M,
\end{equation}
for a constant $\gamma >0$. This completes the proof.
\end{proof}




% \begin{remark}
% For general $M$, only the last part of the proof needs modification. We need $M > T/2 - ck$. For all  $b$ such that $k(b) = |\{i:b_i = 0\}| > T/(2c)- M/c$, the bound \eqref{eq:true-Tp} holds.  In \eqref{eqn:final-line}, we sum over all such $b$'s:
% \begin{align}
%   I(\Pi; C_1,\cdots, C_T)  &\geq   \frac{1}{8}\frac{1}{2^{T}}  \sum_{b  } \sum_{j : b_j = 0} d^2_{\TV} (\Pi_{b \oplus e_j}, \Pi_b) \\
%   & \geq  \frac{1}{8}\frac{1}{2^{T}}  \sum_{b :k(b)> T/2c - M/c} \sum_{j : b_j = 0} d^2_{\TV} (\Pi_{b \oplus e_j}, \Pi_b) \\
%   & \geq \frac{1}{8}\frac{1}{2^{T}}  \sum_{b :k(b) > T/2c - M/c}    \Omega ((1-c)^2 T).
% \end{align}
% \end{remark}





\section{Proof of Theorem \ref{thm:det}}\label{sec:det-pf}

\begin{proof}[Proof of Theorem \ref{thm:det}]
We first remark that the algorithm can make at most $\log k\le\log n$ mistakes over the lifespan of each pool of size $k:=\frac{2nM}{RT}\log n$ because each time the algorithm makes a mistake, at least half of the pool must be incorrect and deleted, so the size of the pool decreases by at least half with each mistake the algorithm mistakes. 

Since each pool $P$ has size $k$ and there are $n$ experts, then there are at most $\frac{2n}{k}$ pools before the entire set $S$, which is initialized to $n$, is depleted. 
Thus, there are at most $\frac{2n}{k}$ pools to iterate through the entire set of experts. 
Moreover, each time the algorithm has iterated through the entire set of experts, each expert must have made at least one mistake. 
This is because an expert is only deleted from the pool $P$ when it has made a mistake and since all experts have been deleted from $P$, then all experts have made at least one mistake. 

Since the best expert makes at most $M$ mistakes, then the best expert can be deleted from the pool $P$ at most $M$ times. 
In other words, the algorithm can cycle through the entire set of $n$ experts at most $M$ times. 

Hence, the total number of mistakes by the algorithm is at most \[\frac{2n}{k}\cdot\log n\cdot M\le\frac{2nRT}{2nM\log n}\cdot\log n\cdot M=RT,\]
so the algorithm achieves regret at most $R$. 
Since the algorithm selects a subset of  $k=\frac{2nM}{RT}\log n$ experts, then the space complexity follows. 
\end{proof}


\section{Proof of Theorem \ref{thm:rand-robust}}\label{sec:rand-robust-pf}
Our algorithm uses a technique introduced by \cite{HassidimKMMS20, attias2021framework,BeimelKMNSS22} to use differential privacy (DP) to hide the internal randomness of our algorithm from an adaptive adversary. 
\begin{proof}[Proof of \autoref{thm:rand-robust}]
Suppose we run $m=\O{\sqrt{T}\log(nT)}$ independent instances of $\discpred$ with regret $\frac{R}{4}$. 
Note that for $R > \frac{64\log^2 n}{T}$, we have $\frac{R}{4}> \frac{16\log^2 n }{T}$, which is a valid input to $\discpred$ in~\autoref{lem:disc:pred}. 
By~\autoref{lem:disc:pred}, each instance succeeds on an arbitrary-order stream with probability at least $1-\frac{1}{\poly(n,T)}$. 
By a union bound over the $m$ instances, all instances succeed with probability at least $1-\frac{1}{\poly(n,T)}$. 
In particular, each instance has regret at most $\frac{R}{4}$, so that the total number of mistakes by each instance is at most $M+\frac{RT}{4}$. 
Thus, the total number of mistakes by all instances is at most $m\left(M+\frac{RT}{4}\right)$. 

To consider an adaptive stream, observe that $\privmed$ is called with privacy parameter $\O{\frac{1}{\sqrt{T}\log(nT)}}$ and failure probability $\frac{1}{\poly(n,T)}$. 
By~\autoref{thm:adaptive:queries}, the mechanism permits $T$ adaptive interactions and guarantees privacy $\O{1}$ with failure probability $\frac{1}{\poly(n,T)}$. 
By~\autoref{thm:generalization}, we have that with high probability, if the output of the algorithm is incorrect, then at least $\frac{m}{3}$ of the instances $\discpred$ are also incorrect. 
Since the total number of mistakes by all instances is at most $m\left(M+\frac{RT}{4}\right)$, then the total number of mistakes by the algorithm is at most $3\left(M+\frac{RT}{4}\right)\le M+RT$, since $M\le\frac{R^2 T}{128\log^2 n}$. 
Hence, the algorithm achieves $R$ regret with high probability. 

By~\autoref{lem:disc:pred}, each instance of $\discpred$ uses $\widetilde{O}\left(\frac{n}{RT}\right)$ space. 
Since we use $$m=\O{\sqrt{T}\log(nT)}$$ independent instances of $\discpred$, then the total space is $\widetilde{O}\left(\frac{n}{R\sqrt{T}}\right)$. 
\end{proof}

